A Large-Scale Study of Probabilistic Calibration in Neural Network Regression

Accurate probabilistic predictions are essential for optimal decision making. While neural network miscalibration has been studied primarily in classification, we investigate this in the less-explored domain of regression. We conduct the largest empirical study to date to assess the probabilistic calibration of neural networks. We also analyze the performance of recalibration, conformal, and regularization methods to enhance probabilistic calibration. Additionally, we introduce novel differentiable recalibration and regularization methods, uncovering new insights into their effectiveness. Our findings reveal that regularization methods offer a favorable tradeoff between calibration and sharpness. Post-hoc methods exhibit superior probabilistic calibration, which we attribute to the finite-sample coverage guarantee of conformal prediction. Furthermore, we demonstrate that quantile recalibration can be considered as a specific case of conformal prediction. Our study is fully reproducible and implemented in a common code base for fair comparisons.

==> tables/calib_nll_real_mixture_1_nb_hidden_1.tex <==
\begin{tabular}{lllll}
	\toprule
	metric & \multicolumn{2}{c}{test\_calib\_l1} & \multicolumn{2}{c}{test\_nll} \\
	model & nn\_no\_regul & qr\_kl\_div & nn\_no\_regul & qr\_kl\_div \\
	dataset &  &  &  &  \\
	\midrule
	airfoil & 0.0423 $\pm$ 0.00072 & \textbf{0.0340 $\pm$ 0.00088} & \textbf{2.33 $\pm$ 0.0036} & 2.34 $\pm$ 0.0044 \\
	concrete & 0.0439 $\pm$ 0.0018 & \textbf{0.0391 $\pm$ 0.0015} & \textbf{3.11 $\pm$ 0.0064} & 3.15 $\pm$ 0.0075 \\
	protein & 0.0413 $\pm$ 0.0012 & \textbf{0.0264 $\pm$ 0.00077} & 2.92 $\pm$ 0.0050 & 2.92 $\pm$ 0.0034 \\
	red & \textbf{0.0324 $\pm$ 0.0019} & 0.0337 $\pm$ 0.0021 & \textbf{0.951 $\pm$ 0.014} & 0.970 $\pm$ 0.016 \\
	diamonds & 0.0408 $\pm$ 0.0028 & \textbf{0.0379 $\pm$ 0.0067} & \textbf{7.88 $\pm$ 0.0039} & 7.92 $\pm$ 0.045 \\
	meps\_19 & 0.132 $\pm$ 0.0012 & \textbf{0.0834 $\pm$ 0.0014} & \textbf{4.07 $\pm$ 0.062} & 4.18 $\pm$ 0.091 \\
	facebook\_1 & 0.103 $\pm$ 0.0010 & \textbf{0.0736 $\pm$ 0.00089} & \textbf{0.715 $\pm$ 0.017} & 0.716 $\pm$ 0.014 \\
	\bottomrule
\end{tabular}

==> tables/calib_nll_real_mixture_3_nb_hidden_3.tex <==
\begin{tabular}{lllll}
	\toprule
	metric & \multicolumn{2}{c}{test\_calib\_l1} & \multicolumn{2}{c}{test\_nll} \\
	model & nn\_no\_regul & qr\_kl\_div & nn\_no\_regul & qr\_kl\_div \\
	dataset &  &  &  &  \\
	\midrule
	airfoil & \textbf{0.0407 $\pm$ 0.0011} & 0.0426 $\pm$ 0.0014 & \textbf{1.81 $\pm$ 0.0064} & 1.92 $\pm$ 0.0071 \\
	concrete & \textbf{0.0459 $\pm$ 0.0025} & 0.0496 $\pm$ 0.0023 & \textbf{3.10 $\pm$ 0.013} & 3.15 $\pm$ 0.012 \\
	protein & \textbf{0.0173 $\pm$ 0.00066} & 0.0205 $\pm$ 0.00088 & \textbf{2.01 $\pm$ 0.0040} & 2.06 $\pm$ 0.0044 \\
	red & 0.0623 $\pm$ 0.0042 & \textbf{0.0596 $\pm$ 0.0047} & -1.63 $\pm$ 0.054 & -1.63 $\pm$ 0.093 \\
	diamonds & 0.0202 $\pm$ 0.0034 & \textbf{0.0164 $\pm$ 0.00093} & \textbf{7.76 $\pm$ 0.0071} & 7.77 $\pm$ 0.0096 \\
	meps\_19 & 0.0424 $\pm$ 0.00065 & \textbf{0.0406 $\pm$ 0.00084} & \textbf{2.65 $\pm$ 0.011} & 2.68 $\pm$ 0.012 \\
	facebook\_1 & 0.114 $\pm$ 0.00060 & \textbf{0.0755 $\pm$ 0.00086} & -1.54 $\pm$ 0.018 & \textbf{-1.48 $\pm$ 0.019} \\
	\bottomrule
\end{tabular}

==> tables/calib_nll_toy_mixture_1_nb_hidden_1.tex <==
\begin{tabular}{lllll}
	\toprule
	metric & \multicolumn{2}{c}{test\_calib\_l1} & \multicolumn{2}{c}{test\_nll} \\
	model & nn\_no\_regul & qr\_kl\_div & nn\_no\_regul & qr\_kl\_div \\
	dataset &  &  &  &  \\
	\midrule
	toy\_1024 & \textbf{0.0314 $\pm$ 0.0027} & 0.0317 $\pm$ 0.0022 & 1.56 $\pm$ 0.014 & \textbf{1.55 $\pm$ 0.011} \\
	toy\_2048 & 0.0257 $\pm$ 0.0042 & \textbf{0.0203 $\pm$ 0.0026} & 1.49 $\pm$ 0.015 & \textbf{1.48 $\pm$ 0.016} \\
	toy\_4096 & 0.0241 $\pm$ 0.0024 & \textbf{0.0158 $\pm$ 0.0021} & 1.48 $\pm$ 0.010 & \textbf{1.47 $\pm$ 0.013} \\
	toy\_8192 & 0.0249 $\pm$ 0.0019 & \textbf{0.0220 $\pm$ 0.0020} & 1.47 $\pm$ 0.0065 & 1.47 $\pm$ 0.013 \\
	toy\_16384 & 0.0296 $\pm$ 0.0024 & \textbf{0.0217 $\pm$ 0.0016} & \textbf{1.46 $\pm$ 0.012} & 1.47 $\pm$ 0.013 \\
	\bottomrule
\end{tabular}


==> tables/calib_nll_toy_mixture_3_nb_hidden_3.tex <==
\begin{tabular}{lllll}
	\toprule
	metric & \multicolumn{2}{c}{test\_calib\_l1} & \multicolumn{2}{c}{test\_nll} \\
	model & nn\_no\_regul & qr\_kl\_div & nn\_no\_regul & qr\_kl\_div \\
	dataset &  &  &  &  \\
	\midrule
	toy\_1024 & 0.0407 $\pm$ 0.0054 & \textbf{0.0394 $\pm$ 0.0078} & \textbf{1.19 $\pm$ 0.026} & 1.22 $\pm$ 0.030 \\
	toy\_2048 & 0.0251 $\pm$ 0.0052 & \textbf{0.0233 $\pm$ 0.0022} & 1.14 $\pm$ 0.015 & 1.14 $\pm$ 0.016 \\
	toy\_4096 & \textbf{0.0226 $\pm$ 0.0025} & 0.0262 $\pm$ 0.0048 & \textbf{1.10 $\pm$ 0.014} & 1.11 $\pm$ 0.017 \\
	toy\_8192 & 0.0200 $\pm$ 0.0014 & \textbf{0.0192 $\pm$ 0.0017} & \textbf{1.12 $\pm$ 0.0070} & 1.13 $\pm$ 0.0077 \\
	toy\_16384 & \textbf{0.0214 $\pm$ 0.0025} & 0.0234 $\pm$ 0.0021 & \textbf{1.11 $\pm$ 0.0087} & 1.12 $\pm$ 0.0091 \\
	\bottomrule
\end{tabular}

==> tables/conformal_tpp.tex <==
\begin{tabular}{llrrrr}
	\toprule
	& & \multicolumn{2}{c}{Coverage} & \multicolumn{2}{c}{Length} \\
	& & Conformal & \makecell{Non \\ conformal} & Conformal & \makecell{Non \\ conformal} \\
	Dataset & Model &  &  &  &  \\
	\midrule
	\multirow[c]{2}{*}{taxi\_reformat} & exponentialconstant & \bfseries 0.94 & 0.83 & 0.56 & \bfseries 0.42 \\
	& lognormmix & 0.78 & \bfseries 1.00 & \bfseries 0.39 & 1.60 \\
	\multirow[c]{2}{*}{yelp\_toronto} & exponentialconstant & \bfseries 0.97 & 0.20 & 2271903.25 & \bfseries 28759.51 \\
	& lognormmix & \bfseries 0.87 & 0.00 & 2076634.25 & \bfseries 17.96 \\
	yelp\_airport\_reformat & lognormmix & \bfseries 0.88 & 1.00 & \bfseries 1.24 & 2.56 \\
	\multirow[c]{2}{*}{yelp\_mississauga\_reformat} & exponentialconstant & \bfseries 0.88 & 0.81 & 0.64 & \bfseries 0.46 \\
	& lognormmix & \bfseries 0.94 & 0.97 & \bfseries 0.89 & 1.49 \\
	\multirow[c]{2}{*}{lastfm\_nomarks} & exponentialconstant & \bfseries 0.92 & 0.78 & 41.59 & \bfseries 15.42 \\
	& lognormmix & \bfseries 0.92 & 0.70 & 45.39 & \bfseries 14.22 \\
	\multirow[c]{2}{*}{wikipedia\_nomarks} & exponentialconstant & \bfseries 0.87 & 0.76 & 88988.45 & \bfseries 44703.18 \\
	& lognormmix & \bfseries 0.90 & 0.05 & 126681.38 & \bfseries 33.38 \\
	\multirow[c]{2}{*}{reddit\_politics\_submissions\_reformat} & exponentialconstant & \bfseries 0.88 & 0.88 & 0.04 & \bfseries 0.04 \\
	& lognormmix & \bfseries 0.95 & 1.00 & \bfseries 0.06 & 0.36 \\
	\multirow[c]{2}{*}{reddit\_askscience\_comments\_reformat} & exponentialconstant & \bfseries 0.85 & 0.77 & 2.20 & \bfseries 1.63 \\
	& lognormmix & \bfseries 0.91 & 0.61 & 2.52 & \bfseries 0.84 \\
	\multirow[c]{2}{*}{twitter\_reformat} & exponentialconstant & \bfseries 0.94 & 0.80 & 4.96 & \bfseries 3.32 \\
	& lognormmix & \bfseries 0.94 & 0.76 & 5.47 & \bfseries 2.98 \\
	\multirow[c]{2}{*}{pubg\_reformat} & exponentialconstant & \bfseries 0.91 & 0.93 & \bfseries 6.04 & 6.32 \\
	& lognormmix & \bfseries 0.91 & 0.97 & \bfseries 2.15 & 3.34 \\
	\multirow[c]{2}{*}{stack\_overflow\_nomarks} & exponentialconstant & 0.90 & \bfseries 0.90 & 1991179.38 & \bfseries 1912994.25 \\
	& lognormmix & \bfseries 0.90 & 0.00 & 1989249.38 & \bfseries 15.23 \\
	\multirow[c]{2}{*}{mooc\_nomarks} & exponentialconstant & \bfseries 0.90 & 0.97 & \bfseries 31191.28 & 46204.48 \\
	& lognormmix & \bfseries 0.90 & 0.36 & 1400.52 & \bfseries 8.09 \\
	\multirow[c]{2}{*}{reddit\_nomarks} & exponentialconstant & \bfseries 0.92 & 0.87 & 134615.47 & \bfseries 92545.35 \\
	& lognormmix & \bfseries 0.88 & 0.01 & 130071.62 & \bfseries 9.68 \\
	hawkes\_exp\_sum & exponentialconstant & \bfseries 0.90 & 0.86 & 1.65 & \bfseries 1.40 \\
	poisson & exponentialconstant & 0.90 & \bfseries 0.90 & 2.34 & \bfseries 2.30 \\
	\bottomrule
\end{tabular}

==> tables/datasets_old.tex <==
\begin{tabular}{lllrrrrr}
	\toprule
	&  &  & \makecell{Nb of \\ features} & \makecell{Nb of \\ training \\ instances} & \makecell{Proportion \\ of duplicated \\ values} & \makecell{Proportion \\ of top 1 \\ class} & \makecell{Proportion \\ of top 10 \\ classes} \\
	Group & Dataset & Abbrev. &  &  &  &  &  \\
	\midrule
	\multirow[t]{11}{*}{uci} & Airfoil & AIR & 5 & 601 & 0.03 & 0.00 & 0.03 \\
	& Concrete & CON & 8 & 412 & 0.08 & 0.01 & 0.06 \\
	& CPU & CP1 & 7 & 83 & \bfseries 0.42 & 0.07 & \bfseries 0.37 \\
	& Crime & CRI & 104 & 326 & \bfseries 0.92 & 0.09 & \bfseries 0.57 \\
	& Energy & ENE & 9 & 307 & 0.15 & 0.01 & 0.08 \\
	& Fish & FIS & 6 & 363 & 0.06 & 0.01 & 0.06 \\
	& MPG & MPG & 7 & 156 & \bfseries 0.67 & 0.04 & \bfseries 0.34 \\
	& Naval & NAV & 17 & 4773 & \bfseries 1.00 & 0.04 & \bfseries 0.41 \\
	& Power & POW & 4 & 3827 & \bfseries 0.49 & 0.00 & 0.01 \\
	& Protein & PRO & 9 & 18292 & \bfseries 0.67 & 0.01 & 0.01 \\
	& Yacht & YAC & 6 & 123 & 0.18 & 0.02 & 0.16 \\
	\multirow[t]{20}{*}{oml\_297} & wine\_quality & WIN & 11 & 2598 & \bfseries 1.00 & \bfseries 0.43 & \bfseries 1.00 \\
	& isolet & ISO & 613 & 3118 & \bfseries 1.00 & 0.05 & \bfseries 0.42 \\
	& cpu\_act & CP2 & 21 & 3276 & \bfseries 1.00 & 0.06 & \bfseries 0.50 \\
	& sulfur & SUL & 6 & 4032 & 0.06 & 0.00 & 0.01 \\
	& Brazilian\_houses & BRA & 8 & 4276 & \bfseries 0.44 & 0.00 & 0.02 \\
	& Ailerons & AIL & 33 & 5500 & \bfseries 1.00 & 0.14 & \bfseries 0.86 \\
	& MiamiHousing2016 & MIA & 13 & 5572 & \bfseries 0.88 & 0.02 & 0.12 \\
	& pol & POL & 26 & 6000 & \bfseries 1.00 & \bfseries 0.62 & \bfseries 0.98 \\
	& elevators & ELE & 16 & 6639 & \bfseries 1.00 & 0.15 & \bfseries 0.79 \\
	& Bike\_Sharing\_Demand & BIK & 6 & 6951 & \bfseries 0.98 & 0.02 & 0.11 \\
	& fifa & FIF & 5 & 7225 & \bfseries 1.00 & 0.16 & \bfseries 0.70 \\
	& houses & HO1 & 8 & 8256 & \bfseries 0.87 & 0.04 & 0.09 \\
	& california & CAL & 8 & 8256 & \bfseries 0.87 & 0.04 & 0.09 \\
	& superconduct & SUP & 79 & 8505 & \bfseries 0.89 & 0.01 & 0.05 \\
	& house\_sales & HO2 & 15 & 8645 & \bfseries 0.84 & 0.01 & 0.07 \\
	& house\_16H & HO3 & 16 & 9113 & \bfseries 0.94 & 0.14 & 0.17 \\
	& diamonds & DIA & 6 & 20000 & \bfseries 0.80 & 0.00 & 0.02 \\
	& medical\_charges & MED & 3 & 20000 & 0.02 & 0.00 & 0.00 \\
	& year & YEA & 90 & 20000 & \bfseries 1.00 & 0.08 & \bfseries 0.58 \\
	& nyc-taxi-green-dec-2016 & NYC & 9 & 20000 & \bfseries 0.99 & 0.15 & \bfseries 0.38 \\
	\multirow[t]{8}{*}{oml\_299} & analcatdata\_supreme & ANA & 12 & 1620 & \bfseries 1.00 & \bfseries 0.70 & \bfseries 1.00 \\
	& \makecell{Mercedes\_Benz\\\_Greener\_Manufacturing} & MER & 735 & 1683 & \bfseries 0.39 & 0.00 & 0.02 \\
	& visualizing\_soil & VIS & 5 & 3456 & \bfseries 1.00 & 0.07 & \bfseries 0.43 \\
	& yprop\_4\_1 & YPR & 82 & 3554 & \bfseries 0.89 & 0.01 & 0.04 \\
	& OnlineNewsPopularity & ONL & 73 & 15857 & \bfseries 0.98 & 0.06 & \bfseries 0.36 \\
	& black\_friday & BLA & 23 & 20000 & \bfseries 0.83 & 0.00 & 0.01 \\
	& \makecell{SGEMM\_GPU\\\_kernel\_performance} & SGE & 15 & 20000 & \bfseries 0.55 & 0.00 & 0.00 \\
	& \makecell{particulate-matter\\-ukair-2017} & PAR & 26 & 20000 & \bfseries 0.89 & 0.01 & 0.06 \\
	\multirow[t]{14}{*}{oml\_269} & tecator & TEC & 124 & 96 & \bfseries 0.35 & 0.03 & \bfseries 0.23 \\
	& boston & BOS & 22 & 202 & \bfseries 0.57 & 0.04 & \bfseries 0.22 \\
	& MIP-2016-regression & MIP & 111 & 436 & 0.12 & 0.01 & 0.06 \\
	& socmob & SOC & 39 & 462 & \bfseries 0.73 & 0.19 & \bfseries 0.36 \\
	& Moneyball & MON & 18 & 492 & \bfseries 0.73 & 0.01 & 0.11 \\
	& house\_prices\_nominal & HO4 & 234 & 437 & \bfseries 0.50 & 0.02 & 0.12 \\
	& us\_crime & US\_ & 101 & 797 & \bfseries 0.98 & 0.05 & \bfseries 0.38 \\
	& quake & QUA & 3 & 871 & \bfseries 1.00 & \bfseries 0.33 & \bfseries 1.00 \\
	& space\_ga & SPA & 6 & 1242 & 0.00 & 0.00 & 0.01 \\
	& abalone & ABA & 10 & 1670 & \bfseries 1.00 & 0.17 & \bfseries 0.90 \\
	& \makecell{SAT11-HAND-\\runtime-regression} & SAT & 118 & 1776 & \bfseries 0.61 & 0.01 & 0.07 \\
	& \makecell{Santander\_transaction\\\_value} & SAN & 3611 & 1783 & \bfseries 0.70 & 0.05 & \bfseries 0.31 \\
	& colleges & COL & 34 & 2678 & \bfseries 0.32 & 0.01 & 0.03 \\
	& topo\_2\_1 & TOP & 252 & 3554 & \bfseries 0.89 & 0.01 & 0.04 \\
	\bottomrule
\end{tabular}

==> tables/improved_test_calib_l2.tex <==
\begin{tabular}{lrrrr}
	\toprule
	nb\_hidden & \multicolumn{2}{r}{1} & \multicolumn{2}{r}{3} \\
	mixture\_size & 1 & 3 & 1 & 3 \\
	\cmidrule(r){1-1}
	model &  &  &  &  \\
	\midrule
	qr\_sorted\_pits\_l1 & 0.77 & 0.42 & 0.77 & 0.42 \\
	qr\_neural\_sorted\_pits\_l1 & 0.84 & 0.61 & 0.71 & 0.61 \\
	qr\_kl\_div & 0.87 & 0.74 & 0.74 & 0.55 \\
	qr\_neural\_sorted\_pits\_l2 & 0.74 & 0.55 & 0.61 & 0.42 \\
	qr\_sorted\_pits\_l2 & 0.71 & 0.55 & 0.65 & 0.58 \\
	qr\_kl\_div\_neural\_sort & 0.94 & 0.61 & 0.81 & 0.55 \\
	qr\_l2 & 0.52 & 0.35 & 0.71 & 0.48 \\
	qr\_l1 & 0.87 & 0.52 & 0.71 & 0.55 \\
	\bottomrule
\end{tabular}

==> tables/improved_test_posthoc_calib_l2.tex <==
\begin{tabular}{lrrrr}
	\toprule
	nb\_hidden & \multicolumn{2}{r}{1} & \multicolumn{2}{r}{3} \\
	mixture\_size & 1 & 3 & 1 & 3 \\
	\cmidrule(r){1-1}
	model &  &  &  &  \\
	\midrule
	qr\_sorted\_pits\_l1 & 0.45 & 0.48 & 0.58 & 0.45 \\
	qr\_neural\_sorted\_pits\_l1 & 0.55 & 0.45 & 0.58 & 0.55 \\
	qr\_kl\_div & 0.65 & 0.68 & 0.58 & 0.29 \\
	qr\_neural\_sorted\_pits\_l2 & 0.48 & 0.39 & 0.52 & 0.45 \\
	qr\_sorted\_pits\_l2 & 0.52 & 0.52 & 0.65 & 0.55 \\
	qr\_kl\_div\_neural\_sort & 0.58 & 0.48 & 0.58 & 0.42 \\
	qr\_l2 & 0.55 & 0.35 & 0.58 & 0.42 \\
	qr\_l1 & 0.48 & 0.65 & 0.55 & 0.32 \\
	\bottomrule
\end{tabular}


==> tables/regularization.tex <==
\begin{tabular}{lllll}
	\toprule
	&  & test\_crps & test\_calib\_l1 & test\_posthoc\_calib\_l1 \\
	Model & L &  &  &  \\
	\midrule
	mixture\_no\_regul & - & 0.252 $\pm$ 0.0055 & 0.102 $\pm$ 0.0039 & 0.0497 $\pm$ 0.0045 \\
	\multirow[t]{2}{*}{mixture\_cdf\_based} & 1 & 0.252 $\pm$ 0.0060 & 0.0857 $\pm$ 0.0045 & 0.0431 $\pm$ 0.0044 \\
	& 2 & 0.255 $\pm$ 0.0086 & 0.0958 $\pm$ 0.0054 & 0.0466 $\pm$ 0.0041 \\
	\multirow[t]{2}{*}{mixture\_quantile\_based} & 1 & 0.254 $\pm$ 0.0072 & 0.0840 $\pm$ 0.0036 & 0.0447 $\pm$ 0.0037 \\
	& 2 & 0.253 $\pm$ 0.0057 & 0.0964 $\pm$ 0.0040 & 0.0464 $\pm$ 0.0034 \\
	mixture\_entropy\_based & - & 0.264 $\pm$ 0.0080 & 0.0657 $\pm$ 0.0051 & 0.0462 $\pm$ 0.0037 \\
	mixture\_ic & - & 0.250 $\pm$ 0.0062 & 0.105 $\pm$ 0.0041 & 0.0428 $\pm$ 0.0044 \\
	mixture\_oqr & - & 1.18 $\pm$ 0.32 & 0.102 $\pm$ 0.0033 & 0.0489 $\pm$ 0.0044 \\
	mixture\_ngboost & - & 0.279 +- 0.0041 & \textbf{0.0591 +- 0.0012} & \textbf{0.00638 +- 0.00071} \\
	quantile\_no\_regul & - & \textbf{0.242 $\pm$ 0.0070} & 0.194 $\pm$ 0.014 & 0.186 $\pm$ 0.013 \\
	\multirow[t]{2}{*}{quantile\_quantile\_based} & 1 & 0.327 $\pm$ 0.0073 & 0.119 $\pm$ 0.0050 & 0.0942 $\pm$ 0.0084 \\
	& 2 & 0.264 $\pm$ 0.0056 & 0.120 $\pm$ 0.0051 & 0.0836 $\pm$ 0.0079 \\
	\bottomrule
\end{tabular}
